Modelling Patient Trajectories Using Multimodal Information

Electronic Health Records (EHRs) aggregate diverse information at the patient level, holding a trajectory representative of the evolution of the patient health status throughout time. Although this information provides context and can be leveraged by physicians to monitor patient health and make more accurate prognoses/diagnoses, patient records can contain information from very long time spans, which combined with the rapid generation rate of medical data makes clinical decision making more complex. Patient trajectory modelling can assist by exploring existing information in a scalable manner, and can contribute in augmenting health care quality by fostering preventive medicine practices. We propose a solution to model patient trajectories that combines different types of information and considers the temporal aspect of clinical data. This solution leverages two different architectures: one supporting flexible sets of input features, to convert patient admissions into dense representations; and a second exploring extracted admission representations in a recurrent-based architecture, where patient trajectories are processed in sub-sequences using a sliding window mechanism. The developed solution was evaluated on two different clinical outcomes, unexpected patient readmission and disease progression, using the publicly available MIMIC-III clinical database. The results obtained demonstrate the potential of the first architecture to model readmission and diagnoses prediction using single patient admissions. While information from clinical text did not show the discriminative power observed in other existing works, this may be explained by the need to fine-tune the clinicalBERT model. Finally, we demonstrate the potential of the sequence-based architecture using a sliding window mechanism to represent the input data, attaining comparable performances to other existing solutions.

==> Modelling_Patient_Trajectories_Using_Multimodal_Information - preprint/Tabs/hadm_distribution.tex <==
\begingroup
\renewcommand{\arraystretch}{0.9}
\begin{table}[!h]
\centering
\caption[Dataset distributions for the readmission prediction and diagnosis prediction tasks.]{Dataset distributions for the readmission prediction and diagnosis prediction tasks, obtained using stratified distribution at the patient level. Values reported in Fold columns correspond to the number of admissions present in each fold.}
\label{tab:chap5:hadm_distribution}
\begin{tabular}{cc@{}c@{}cccccccccc@{}c@{}}
\toprule
&  &  &  & \multicolumn{10}{c}{Fold} \\
Task & & Label & & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
\cmidrule{1-1}\cmidrule{3-3}\cmidrule{5-14}
\multirow{2}{*}{Readmission} & & 0 & & 4128 & 4228 & 4018 & 4091 & 4136 & 4124 & 4079 & 4049 & 4053 & 4066 \\
& & 1 & & 280 & 323 & 264 & 285 & 281 & 297 & 276 & 306 & 288 & 307 \\
\cmidrule{3-3}\cmidrule{5-14} 
Diagnosis & & --- & & \multicolumn{1}{l}{1073} & \multicolumn{1}{l}{1200} & \multicolumn{1}{l}{939} & \multicolumn{1}{l}{1014} & \multicolumn{1}{l}{1064} & \multicolumn{1}{l}{1079} & \multicolumn{1}{l}{990} & \multicolumn{1}{l}{1011} & \multicolumn{1}{l}{990} & \multicolumn{1}{l}{1016} \\
\bottomrule
\end{tabular}
\end{table}

\endgroup

==> Modelling_Patient_Trajectories_Using_Multimodal_Information - preprint/Tabs/hadm_distribution_hadmsplit.tex <==
\begingroup
\renewcommand{\arraystretch}{0.9}
\begin{table}[!h]
\centering
\caption[Dataset distribution for the readmission prediction task, with stratified distribution at the admission level.]{Dataset distribution for the readmission prediction task, with stratified distribution at the admission level. Values reported in Fold columns correspond to the number of admissions present in each fold.}
\label{tab:chap5:hadm_distribution_hadmsplit}
\begin{tabular}{cc@{}c@{}ccccccccccc@{}}
\toprule
&  &  &  & \multicolumn{10}{c}{Fold} \\
Task & & Label & & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
\cmidrule{1-1}\cmidrule{3-3}\cmidrule{5-14}
\multirow{2}{*}{Readmission} & & 0 & & 4091 & 4106 & 4086 & 4106 & 4083 & 4123	& 4093 & 4099 & 4090 & 4095 \\
& & 1 & & 291 &  292 &  291 &  292 &  291 &  289	&  291 &  289 &  291 &  290 \\
\bottomrule
\end{tabular}
\end{table}

\endgroup



==> Modelling_Patient_Trajectories_Using_Multimodal_Information - preprint/Tabs/hyperparams_individual.tex <==
\begingroup
\renewcommand{\arraystretch}{1.2}
\begin{table}[!t]
\centering
\caption[List of~\textquotedblleft optimal\textquotedblright~hyperparameters used for training the first model architecture.]{List of~\textquotedblleft optimal\textquotedblright~hyperparameters used for training the first model architecture. RP: readmission prediction, DP: diagnoses prediction.}
\label{tab:chap5:hyperparameters_individualmodel}
\begin{tabular}{ccc}
\toprule
Description & & Value \\
\cmidrule{1-1}\cmidrule{3-3}

Dimension of clinicalBERT embeddings & & 768\\
Dimension of SapBERT embeddings & & 768\\
Hidden layer size (temporal features) & & 50 \\
Dropout rate & & 0.1\\
Activation function & & Mish\\
Subsampling & & RP: True | DP: False\\
%\multirow{2}{*}{Subsampling} & & Readmission: True\\
%& & Diagnoses: False\\
Train batch size & & 64\\
Number of training epochs & & 100\\
Learning rate & & 0.001\\
Early stop & & True\\
Number of patience steps & & 200\\
Optimizer & & Ranger\\

\bottomrule
\end{tabular}
\end{table}
\endgroup



==> Modelling_Patient_Trajectories_Using_Multimodal_Information - preprint/Tabs/hyperparams_trajectory.tex <==
\begingroup
\renewcommand{\arraystretch}{1.2}
\begin{table}[!h]
\centering
\caption[List of experimental hyperparameters for training the second model architecture.]{List of experimental hyperparameters used for training the second model architecture.}% RP: readmission prediction, DP: diagnoses prediction.}
\label{tab:chap5:hyperparameters_trajectorymodel}
\begin{tabular}{ccc}
\toprule
Description & & Value \\
\cmidrule{1-1}\cmidrule{3-3}
Type of recurrent network & & \{GRU, LSTM\}\\
Hidden layer size (recurrent network) & & \{255,~818\}\\
Number of layers (recurrent network) & & \{1,~2,~3\}\\
Bidirectionality & & \{True, False\} \\
Dropout rate & & 0.2\\
Admissions in sliding window & & \{3,~6\}\\
%Subsampling & & RP: \textbf{TESTING} | DP: False\\
Train batch size & & 64\\
Number of training epochs & & 200\\
Learning rate & & 0.001\\
Early stop & & True\\
Number of patience steps & & 200\\
Optimizer & & Ranger\\

\bottomrule
\end{tabular}
\end{table}
\endgroup



==> Modelling_Patient_Trajectories_Using_Multimodal_Information - preprint/Tabs/results_diagnosis_ccs.tex <==
\begingroup
\renewcommand{\arraystretch}{0.95}
\begin{table}[!ht]
\centering
\caption[Diagnoses prediction results (CCS codes) for the individual admission model architecture.]{Diagnoses prediction results (CCS codes) for the individual admission model architecture. Results reported for 10-fold cross-validation. Micro values presented for AU-PR, $F_1$-score and RP80. Best values for each metric highlighted in bold.}
\label{tab:chap5:results_individual_diagnosis_ccs}
\begin{tabular}{@{}lc cccccc@{}}%lclcC{3.3cm}C{3.3cm}C{3.3cm}}
\toprule
Features & & AU-PR & $F_1$-score & RP80 & Recall@10 & Recall@20 &Recall@30 \\
\cmidrule{1-1}\cmidrule{3-8}
Text  & & 0.281 & 0.058 & 0.001 & 0.299 & 0.471 & 0.598 \\
Diag CCS & & 0.437 & 0.320 & 0.101 & 0.417 & 0.583 & 0.686 \\
Text + Diag CCS & & \textbf{0.444} & \textbf{0.346} & 0.104 & \textbf{0.426} & \textbf{0.597} & \textbf{0.699} \\
Diag CCS + Days to prior admission & & 0.439 & 0.323 & \textbf{0.107} & 0.421 & 0.591 & 0.694 \\
Text + Diag CCS + CUI & & 0.425 & 0.299 & 0.090 & 0.406 & 0.576 & 0.680 \\
Text + Diag CCS + Proc CCS  & & 0.431 & 0.315 & 0.094 & 0.413 & 0.583 & 0.686 \\
Text + Diag CCS + Days to prior admission & & 0.426 & 0.306 & 0.091 & 0.407 & 0.579 & 0.682 \\
Text + Diag CCS + Days to prior admission + Proc CCS  & & 0.433 & 0.321 & 0.101 & 0.415 & 0.585 & 0.687 \\
%Text + Diag CCS + Days to prior admission + CUI & & 0.426 & 0.304 & 0.096 & 0.407 & 0.578 & 0.682 \\
Text + Diag CCS + Days to prior admission + Proc CCS + CUI & & 0.429 & 0.322 & 0.095 & 0.412 & 0.583 & 0.685 \\
\cmidrule{1-1}\cmidrule{3-8}
ClinicalBERT\_multi~\cite{franz2020DeepObserver} --- Text & & 0.408 & --- & 0.081 & --- & --- & --- \\
LIG-Doctor~\cite{LIGDoctor2020} --- Diag CCS & & --- & --- & --- & 0.520 & 0.680 & 0.760 \\
\bottomrule
\end{tabular}
\end{table}
\endgroup

==> Modelling_Patient_Trajectories_Using_Multimodal_Information - preprint/Tabs/results_diagnosis_icd.tex <==
\begingroup
\renewcommand{\arraystretch}{0.95}
\begin{table}[!th]
\centering
\caption[Diagnoses prediction results (ICD-9 codes) for the individual admission model architecture.]{Diagnoses prediction results (ICD-9 codes) for the individual admission model architecture. Results reported for 10-fold cross-validation. Micro values presented for AU-PR, $F_1$-score and RP80. Best values for each metric highlighted in bold.}
\label{tab:chap5:results_individual_diagnosis_icd}
\begin{tabular}{@{}lc @{}cccccc@{}}%lclcC{3.3cm}C{3.3cm}C{3.3cm}}
\toprule
Features & & AU-PR & $F_1$-score & RP80 & Recall@10 & Recall@20 &Recall@30 \\
\cmidrule{1-1}\cmidrule{3-8}
Text  & & 0.241 & 0.004 & 0.001 & 0.277 & 0.417 & 0.509 \\
Diag ICD9 & & 0.364 & 0.258 & 0.086 & 0.356 & 0.496 & 0.584 \\
Text + Diag ICD9 & & 0.365 & 0.293 & 0.083 & 0.361 & 0.498 & 0.584 \\
Diag ICD9 + Days to prior admission & & 0.367 & 0.283 & \textbf{0.088} & 0.358 & 0.502 & 0.588 \\
Text + Diag ICD9 + CUI & & 0.357 & 0.254 & 0.077 & 0.346 & 0.487 & 0.576 \\
Text + Diag ICD9 + Proc ICD9  & & 0.362 & 0.262 & 0.079 & 0.351 & 0.493 & 0.582 \\
Text + Diag ICD9 + Days to prior admission & & \textbf{0.370} & \textbf{0.316} & 0.083 & \textbf{0.365} & \textbf{0.506} & \textbf{0.590} \\
Text + Diag ICD9 + Days to prior admission + Proc ICD9  & & 0.362 & 0.270 & 0.082 & 0.352 & 0.494 & 0.582 \\
%Text + Diag ICD9 + Days to prior admission + CUI & & 0.359 & 0.254 & 0.083 & 0.347 & 0.490 & 0.576 \\
Text + Diag ICD9 + Days to prior admission + Proc ICD9 + CUI & & 0.364 & 0.266 & 0.086 & 0.353 & 0.496 & 0.584 \\
\cmidrule{1-1}\cmidrule{3-8}
LIG-Doctor~\cite{LIGDoctor2020} --- Diag ICD9 & & --- & --- & --- & 0.420 & 0.580 & 0.670 \\
\bottomrule
\end{tabular}
\end{table}
\endgroup

==> Modelling_Patient_Trajectories_Using_Multimodal_Information - preprint/Tabs/results_readmission.tex <==
\begingroup
\renewcommand{\arraystretch}{1.0}
\begin{table}[!ht]
\centering
\caption[Final readmission prediction results for the individual admission model architecture.]{Final readmission prediction results for the individual admission model architecture. Results reported for 10-fold cross-validation. ClinicalBERT results presented for comparison. Best results highlighted in bold.}
\label{tab:chap5:results_individual_readmission}
\begin{tabular}{lc cccccc}%lclcC{3.3cm}C{3.3cm}C{3.3cm}}
\toprule
Features & & AUC & AU-PR & $F_1$-score & Precision & Recall & RP80\\
\cmidrule{1-1}\cmidrule{3-8}
Text  & & 0.795 & 0.363 & 0.717 & 0.680 & 0.759 & 0.001 \\
Duration & & 0.567 & 0.521 & 0.517 & 0.553 & 0.492 & 0.050 \\
Days to prior admission & & 0.797 & 0.739 & 0.822 & 0.737 & 0.931 & 0.373 \\
Text + Duration & & 0.794 & 0.360 & 0.719 & 0.680 & 0.762 & 0.001 \\
Days to prior admission + Text & & \textbf{0.871} & 0.468 & 0.820 & \textbf{0.766} & 0.881 & 0.001 \\
Days to prior admission + Duration & & 0.791 & \textbf{0.750} & \textbf{0.828} & 0.737 & \textbf{0.945} & \textbf{0.481} \\
Days to prior admission + Duration + Text & & 0.869 & 0.473 & 0.821 & \textbf{0.766} & 0.885 & 0.001 \\
Days to prior admission + Duration + Text + Diag ICD9 & & 0.773 & 0.440 & 0.739 & 0.733 & 0.754 & 0.001 \\
\cmidrule{1-1}\cmidrule{3-8}
ClinicalBERT~\cite{clinicalBERT2020} --- Text & & 0.714 & 0.701 & --- & --- & --- & 0.242 \\ 
\bottomrule
\end{tabular}
\end{table}
\endgroup

==> Modelling_Patient_Trajectories_Using_Multimodal_Information - preprint/Tabs/results_readmission_experiments1.tex <==
%\begingroup
%\renewcommand{\arraystretch}{1.0}
%\begin{table}[!th]
%\centering
%\caption{Readmission prediction results for the individual admission model architecture, using fine-tuned clinicalBERT and a 5-fold version of the dataset from~\cite{clinicalBERT2020}. Results reported for 5-fold cross validation.}
%\label{tab:chap5:results_individual_readmission_experiments1}
%\begin{tabular}{lc cccccc}%lclcC{3.3cm}C{3.3cm}C{3.3cm}}
%\toprule
%Features & & AUC & AU-PR & $F_1$-score & Precision & Recall & RP80\\
%\cmidrule{1-1}\cmidrule{3-8}
%Text & & 0.829 & 0.804 & 0.719 & 0.686 & 0.755 & 0.614 \\
%Duration & & 0.611 & 0.581 & 0.504 & 0.531 & 0.482 & 0.025 \\
%Days to prior admission & & 0.810 & 0.712 & 0.836 & 0.718 & 0.999 & 0.033 \\
%Duration + Days to prior admission & & 0.864 & 0.780 & 0.836 & 0.718 & 0.999 & 0.238 \\	
%Text + Duration + Days to prior admission & & 0.914 & 0.890 & 0.849 & 0.761 & 0.959 & 0.904\\
%\bottomrule
%\end{tabular}
%\end{table}
%\endgroup


\begingroup
\renewcommand{\arraystretch}{1.0}
\begin{table}[!th]
\centering
\caption[Experimental readmission prediction results for the individual admission model architecture, using fine-tuned clinicalBERT with a 5-fold version of the dataset from clinicalBERT.]{Experimental readmission prediction results for the individual admission model architecture, using fine-tuned clinicalBERT with a 5-fold version of the dataset from~\cite{clinicalBERT2020}, and pretrained clinicalBERT with the new 10-fold dataset. Best results in bold.}
\label{tab:chap5:results_individual_readmission_experiments1}
\begin{tabular}{clc cccccc@{}}%lclcC{3.3cm}C{3.3cm}C{3.3cm}}
\toprule
Resources & Features & & AUC & AU-PR & $F_1$-score & Precision & Recall & RP80\\
\cmidrule{1-2}\cmidrule{4-9}
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Finetuned\\clinicalBERT\\ + \\ 5-fold original \\ dataset\end{tabular}} & Text & & 0.829 & 0.804 & 0.719 & 0.686 & 0.755 & 0.614 \\
 & Duration & & 0.611 & 0.581 & 0.504 & 0.531 & 0.482 & 0.025 \\
 & Days to prior admission & & 0.810 & 0.712 & 0.836 & 0.718 & \textbf{0.999} & 0.033 \\
 & Days to prior admission + Duration & & 0.864 & 0.780 & 0.836 & 0.718 & \textbf{0.999} & 0.238 \\	
 & Days to prior admission + Duration + Text & & \textbf{0.914} & \textbf{0.890} & \textbf{0.849} & \textbf{0.761} & 0.959 & \textbf{0.904}\\
\cmidrule{1-2}\cmidrule{4-9}
\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}Pretrained\\clinicalBERT + \\ 10-fold new \\ dataset\end{tabular}} & Text & & 0.822 & 0.403 & 0.713 & 0.683 & 0.747 & 0.001 \\		
& Duration & & 0.549 & 0.468 & 0.367 & 0.316 & 0.481 & 0.011 \\
& Days to prior admission & & 0.798 & 0.731 & 0.844 & 0.730 & 0.999 & 0.082 \\		
%& Text + Duration & & 0.818 & 0.394 & 0.711 & 0.685 & 0.740 & 0.001 \\	
& Days to prior admission + Text & & 0.885 & 0.504 & \textbf{0.845} & 0.756 & \textbf{0.957} & 0.001 \\	
& Days to prior admission + Duration & & 0.788 & \textbf{0.761} & 0.805 & 0.730 & 0.898 & \textbf{0.358} \\		
& Days to prior admission + Duration + Text  & & \textbf{0.889} & 0.502 & \textbf{0.845} & \textbf{0.757} & 0.955 & 0.002 \\
\bottomrule
\end{tabular}
\end{table}
\endgroup

==> Modelling_Patient_Trajectories_Using_Multimodal_Information - preprint/Tabs/results_readmission_experiments2.tex <==
\begingroup
\renewcommand{\arraystretch}{1.0}
\begin{table}[!ht]
\centering
\caption{Readmission prediction results for the individual admission model architecture, using pretrained clinicalBERT and a 10-fold stratified dataset with selected data from~\gls{mimic}-III (data distributed into folds with splitting at the admission level). Results reported for 10-fold cross validation.}
\label{tab:chap5:results_individual_readmission_experiments2}
\begin{tabular}{lc cccccc}%lclcC{3.3cm}C{3.3cm}C{3.3cm}}
\toprule
Features & & AUC & AU-PR & $F_1$-score & Precision & Recall & RP80\\
\cmidrule{1-1}\cmidrule{3-8}
Text & & 0.822 & 0.403 & 0.713 & 0.683 & 0.747 & 0.001 \\		
Duration & & 0.549 & 0.468 & 0.367 & 0.316 & 0.481 & 0.011 \\
Days to prior admission & & 0.798 & 0.731 & 0.844 & 0.730 & 0.999 & 0.082 \\		
Text + Duration & & 0.818 & 0.394 & 0.711 & 0.685 & 0.740 & 0.001 \\	
Text + Days to prior admission & & 0.885 & 0.504 & 0.845 & 0.756 & 0.957 & 0.001 \\	
Duration + Days to prior admission & & 0.788 & 0.761 & 0.805 & 0.730 & 0.898 & 0.358 \\		
Text + Duration + Days to prior admission & & 0.889 & 0.502 & 0.845 & 0.757 & 0.955 & 0.002 \\	
\bottomrule
\end{tabular}
\end{table}
\endgroup

==> Modelling_Patient_Trajectories_Using_Multimodal_Information - preprint/Tabs/results_trajectory_multihot.tex <==
\begingroup
\renewcommand{\arraystretch}{0.95}
\begin{table}[!th]
\centering
\caption[Preliminary results for diagnoses prediction (CCS codes) using the admission sequence-based model architecture with multi-hot diagnoses input.]{Preliminary results for diagnoses prediction (CCS codes) using the admission sequence-based model architecture with multi-hot diagnoses input. Average results reported for 10-fold cross-validation. Micro values presented for AU-PR, $F_1$-score and RP80. Best values for each metric are highlighted in bold.}
\label{tab:chap5:results_trajectory_diagnosis_multihot_ccs}
\begin{tabular}{cccccc cccccc}%lclcC{3.3cm}C{3.3cm}C{3.3cm}}
\toprule
\begin{tabular}[c]{@{}c@{}}Layer\\Type\end{tabular} & \begin{tabular}[c]{@{}c@{}}Layer\\Size\end{tabular} & \begin{tabular}[c]{@{}c@{}}Num\\Layers\end{tabular} & Bidirectional & \begin{tabular}[c]{@{}c@{}}Sliding \\Window \end{tabular} & & AU-PR & $F_1$-score & RP80 & Recall@10 & Recall@20 &Recall@30 \\
\cmidrule{1-5}\cmidrule{7-12}
GRU	 & 255 & 1 & False & 3 & & 0.466 & 0.324 & 0.123 & 0.433 & 0.605 & 0.707 \\
GRU	 & 255 & 1 & True  & 3 & & \textbf{0.503} & \textbf{0.400} & 0.153 & \textbf{0.464} & \textbf{0.638} & \textbf{0.736} \\
GRU	 & 255 & 1 & True  & 6 & & 0.486 & 0.377 & 0.137 & 0.456 & 0.627 & 0.726 \\
GRU	 & 255 & 2 & True  & 3 & & 0.492 & 0.392 & \textbf{0.157} & 0.454 & 0.627 & 0.726 \\
GRU	 & 255 & 2 & True  & 6 & & 0.478 & 0.372 & 0.142 & 0.448 & 0.619 & 0.718 \\
LSTM & 255 & 1 & True  & 3 & & 0.478 & 0.353 & 0.125 & 0.442 & 0.614 & 0.715 \\
LSTM & 255 & 1 & True  & 6 & & 0.458 & 0.319 & 0.107 & 0.431 & 0.601 & 0.704 \\
\cmidrule{1-5}\cmidrule{7-12}
\begin{tabular}[c]{@{}c@{}}MGRU\\(LIG-Doctor~\cite{LIGDoctor2020})\end{tabular} & 271 & 1 & True & -- & & --- & --- & --- & 0.520 & 0.680 & 0.760 \\
\bottomrule
\end{tabular}
\end{table}
\endgroup

==> Modelling_Patient_Trajectories_Using_Multimodal_Information - preprint/Tabs/results_trajectory_preliminary.tex <==
\begingroup
\renewcommand{\arraystretch}{0.95}
\begin{table}[!th]
\centering
\caption[Preliminary results for diagnoses prediction (CCS codes) using the admission sequence-based model architecture.]{Preliminary results for diagnoses prediction (CCS codes) using the admission sequence-based model architecture. Results reported for 10-fold cross-validation. Micro values presented for AU-PR, $F_1$-score and RP80. Best values highlighted in bold.}
\label{tab:chap5:results_trajectory_diagnosis_ccs}
\begin{tabular}{cccccc cccccc}%lclcC{3.3cm}C{3.3cm}C{3.3cm}}
\toprule
\begin{tabular}[c]{@{}c@{}}Layer\\Type\end{tabular} & \begin{tabular}[c]{@{}c@{}}Layer\\Size\end{tabular} & \begin{tabular}[c]{@{}c@{}}Num\\Layers\end{tabular} & Bidirectional & \begin{tabular}[c]{@{}c@{}}Sliding \\Window \end{tabular} & & AU-PR & $F_1$-score & RP80 & Recall@10 & Recall@20 &Recall@30 \\
\cmidrule{1-5}\cmidrule{7-12}

LSTM & 255 & 1 & False & 3 & & 0.109 & 0.099 & 0.001 & 0.212 & 0.353 & 0.467 \\
LSTM & 255 & 1 & True  & 3 & & 0.127 & 0.129 & 0.001 & 0.223 & 0.366 & 0.473 \\
LSTM & 818 & 1 & True  & 3 & & 0.137 & 0.156 & 0.001 & 0.206 & 0.350 & 0.462 \\
LSTM & 818 & 1 & True  & 6 & & 0.132 & 0.152 & 0.001 & 0.209 & 0.351 & 0.462 \\
LSTM & 255 & 2 & True  & 3 & & 0.134 & 0.182 & 0.001 & 0.234 & 0.399 & 0.522 \\
LSTM & 818 & 2 & True  & 3 & & \textbf{0.174} &	\textbf{0.212} & 0.001 & \textbf{0.245} & \textbf{0.408} & \textbf{0.531} \\
LSTM & 818 & 2 & True  & 6 & & 0.165 &	0.206 & 0.001 &	0.241 &	\textbf{0.408} & \textbf{0.531} \\
LSTM & 818 & 3 & True  & 3 & & 0.117 &	0.149 & 0.001 &	0.232 &	0.407 & \textbf{0.531} \\
GRU  & 818 & 2 & True  & 3 & & 0.138 &	0.204 & 0.001 &	0.224 &	0.381 & 0.502 \\
\bottomrule
\end{tabular}
\end{table}
\endgroup

==> Tabs/results_readmission_experiments2.tex <==
\begingroup
\renewcommand{\arraystretch}{1.0}
\begin{table}[!ht]
\centering
\caption{Readmission prediction results for the individual admission model architecture, using pretrained clinicalBERT and a 10-fold stratified dataset with selected data from~\gls{mimic}-III (data distributed into folds with splitting at the admission level). Results reported for 10-fold cross validation.}
\label{tab:chap5:results_individual_readmission_experiments2}
\begin{tabular}{lc cccccc}%lclcC{3.3cm}C{3.3cm}C{3.3cm}}
\toprule
Features & & AUC & AU-PR & $F_1$-score & Precision & Recall & RP80\\
\cmidrule{1-1}\cmidrule{3-8}
Text & & 0.822 & 0.403 & 0.713 & 0.683 & 0.747 & 0.001 \\		
Duration & & 0.549 & 0.468 & 0.367 & 0.316 & 0.481 & 0.011 \\
Days to prior admission & & 0.798 & 0.731 & 0.844 & 0.730 & 0.999 & 0.082 \\		
Text + Duration & & 0.818 & 0.394 & 0.711 & 0.685 & 0.740 & 0.001 \\	
Text + Days to prior admission & & 0.885 & 0.504 & 0.845 & 0.756 & 0.957 & 0.001 \\	
Duration + Days to prior admission & & 0.788 & 0.761 & 0.805 & 0.730 & 0.898 & 0.358 \\		
Text + Duration + Days to prior admission & & 0.889 & 0.502 & 0.845 & 0.757 & 0.955 & 0.002 \\	
\bottomrule
\end{tabular}
\end{table}
\endgroup
